AI-Resilient Interfaces

AI is powerful, but it can make choices that result in objective errors, contextually inappropriate outputs, and disliked options. We need AI-resilient interfaces that help people be resilient to the AI choices that are not right, or not right for them. To support this goal, interfaces need to help users notice and have the context to appropriately judge those AI choices. Existing human-AI interaction guidelines recommend efficient user dismissal, modification, or otherwise efficient recovery from AI choices that a user does not like. However, in order to recover from AI choices, the user must notice them first. This can be difficult. For example, when generating summaries of long documents, a system's exclusion of a detail that is critically important to the user is hard for the user to notice. That detail can be hiding in a wall of text in the original document, and the existence of a summary may tempt the user not to read the original document as carefully. Once noticed, judging AI choices well can also be challenging. The interface may provide very little information that contextualizes the choices, and the user may fall back on assumptions when deciding whether to dismiss, modify, or otherwise recover from an AI choice. Building on prior work, this paper defines key aspects of AI-resilient interfaces, illustrated with examples. Designing interfaces for increased AI-resilience of users will improve AI safety, usability, and utility. This is especially critical where AI-powered systems are used for context- and preference-dominated open-ended AI-assisted tasks, like ideating, summarizing, searching, sensemaking, and the reading and writing of text or code.

==> other-content-to-consider.tex <==

\section{Not sure where this goes}
Many AI systems must choose between many possible outputs that are all consistent with the user's explicit request, such as identifying relevant case law, Excel's macro-by-example feature~\cite{gulwani2011automating}, and recommender systems.
%inferred to be desirable given data reflecting the user's implicit preferences (e.g., recommendation engines).
%\footnote{It is possible to have multiple distinct possible outputs that are all consistent with the user-provided specification because almost all user specifications are partial; any human is, for almost any non-trivial challenge, incapable of knowing and clearly communicating a complete specification in a non-ambiguous way.} 
This presents an extension of the Invisible AI Choice issue.
\textit{If the user cannot see} any information about 
%unrecommended options or 
the outputs the AI did not choose, \textit{they are unable to judge} whether the AI's ranking method accurately captures what they situationally care about,
%and the situation they are in,
%\footnote{In other words, they do not know enough of the context to accurately judge whether they agree with the AI's choice.} 
and \textit{they are unable to recover} from any mismatch. Note that traditional search interfaces \textit{still} deliver results as a nearly infinite list of pages that are less and less highly ranked, given that the user's explanation of what they want and the ranking algorithm can both imperfectly reflect what the user is looking for, and the user can either continue down the list farther and farther or adjust their query. This is a more AI-resilient interface than interfaces that only show the top 1 or top-$K$ results for some relatively limited $K$.
%a ranking function that poorly captures their context, values, goals, and preferences.
They are also more likely to fall victim to anchoring bias~\cite{kahnemanandtversky} and design fixation based on what outputs they do see~\cite{dow2010parallel}.

\section{More stuff from earlier}
Perfect agreement with user beliefs and preferences right now may also not best serve the user. 
\cite{antagonisticAI} 
We argue that the best outcome is for the user to arrive at, with or without AI assistance, outcomes that would still be
deemed appropriate by the user even if they spent unlimited additional time on the task. 

Seeing a particular AI output can help or hinder the user's arrival at that best outcome: it may serve as an intent elicitation mechanism for the user, helping them recognize, refine, or entirely revise what they want~\cite{ragae} or cause them to fixate/anchor~\cite{kahnemanandtversky} on the option(s) that depend on or are nearby to that particular AI output.\footnote{Seeing multiple outputs may mitigate some but not all of this anchoring effects.}

And as the user's intent evolves and possibly solidifies during their interaction with the system, so may their definition of which AI-made choices are user context \& preference-specific AI errors. For example, the judge may realize that a particular detail they would normally have ignored in the full court document is, in that case, 
critical to consider and 
important to preserve in the summary. 

error status of each AI-made choice.
, creating new instances of this kind of error during the user's interaction with the system. 
as the user creating this kind of error in the moment of that user's recognition. 
an important aspect of utility for interactive systems, 

\section{More text that was commented out of the Google proposal}

\noindent\textbf{In summary,} given AI's new capabilities to handle open-ended tasks in nuanced situations (where users have significant relevant but only partially observable knowledge, context, preferences, goals, and values), we believe that objective correctness is not a well-defined or appropriate goal. We argue that a system that aims primarily for some definition of accuracy\footnote{(even if accuracy is defined by distance to the outcome the user would hypothetically have arrived at, with or without AI assistance, after working on the task with unlimited time and attention)} is a recipe for poor usability and utility.
It puts the user at risk for both walking away with a worse outcome than they theoretically could have had\footnote{due to missing, possibly necessary intent-refining insights triggered by contemplation of AI-generated alternatives} while also being confidently wrong about the appropriateness of the AI's assistance.\footnote{Just as the AI can be confidently wrong about what is most appropriate for the user, the user can be confidently wrong about the appropriateness of the AI's assistance.}

Since only the user can definitively identify user-specific AI errors, inattentional blindness is a significant barrier to a user noticing and recovering from such errors in the moment (to ideally perform their primary task as well as if the AI had not made this error) or by providing feedback that contributes to the longer-term training of better models. This concern applies to some types of objective errors as well. 
personalization or training of better models. 
or better overall training of such models for future .
an AI choice about its output 

the focus on defining objectively \textit{correct} outputs is no longer the right frame,  because it captures objective errors like confabulations but not errors defined by whether that output \textit{agrees} with what that particular user needs or wants in that context for that task. Since only the user can identify such errors, and the only way they can determine that they \textit{disagree} with the AI's choice is if they notice it.\footnote{To complicate matters further, the user (1) may not now (or ever) consciously have a full understanding of what they want, (2) what they want may change as their mental model of the system and their context evolve, and regardless of how complete their understanding of their potentially evolving desires, (3) it may not be easy or possible for them to clearly externalize what they want to the system, e.g., through iterative careful prompt experimentation and tuning\cite{chainforge} or by composing small sets of examples with annotations about how the system should generalize from them\cite{ragae}.}  
Given that the person is not also doing the task themselves, collecting training data from that person's prior interactions with a system will  
Given how much of the user's notion of an appropriate output is conditioned on partially or unobservable values, preferences, context, and goals, we believe continuing to almost exclusively focus on developing more ``accurate'' AI-backed interfaces is a fool's errand.\footnote{More specifically, it is our position that improving the average quality of the AI will always be worthwhile, but, given that guessing more and more accurately what the user wants in these open-ended tasks would eventually require mind-reading.} 
given the quality and pervasiveness of AI-backed systems already being deployed on these open-ended tasks,


Given that the AI and the user may not yet agree on the most appropriate output---at times often or even most of the time---designing for 

with the assumption that the user will often agreement with what the user considers the best and most appropriate output is a fool's errand. In 

and while both lay users and domain experts can encounter them when receving automated assistance, the risks to both AI safety and utility are especially apparent in the latter case. 
This poses risks to both AI safety and utility. 
%While writing may, on the surface, have little to do with 
